Batch Policy Learning under Constraints

When learning policies for real-world domains, two important questions arise: (i) how to efficiently use pre-collected off-policy, non-optimal behavior data; and (ii) how to mediate among different competing objectives and constraints. We thus study the problem of batch policy learning under multiple constraints, and offer a systematic solution. We first propose a flexible meta-algorithm that admits any batch reinforcement learning and online learning procedure as subroutines. We then present a specific algorithmic instantiation and provide performance guarantees for the main objective and all constraints. To certify constraint satisfaction, we propose a new and simple method for off-policy policy evaluation (OPE) and derive PAC-style bounds. Our algorithm achieves strong empirical results in different domains, including in a challenging problem of simulated car driving subject to multiple constraints such as lane keeping and smooth driving. We also show experimentally that our OPE method outperforms other popular OPE techniques on a standalone basis, especially in a high-dimensional setting.

==> sec-proof-fqi.tex <==
%!TEX root = icml_paper.tex
\section{Finite-Sample Analysis of Fitted Q Iteration (FQI)}
\label{sec:proof-fqi}
\subsection{FQI Pseudo-Code and Discussion}
%\subsection{Fitted Q Iteration}
\begin{algorithm}[H]
    \begin{small}
    \caption{ Fitted Q Iteration with Function Approximation: $\texttt{FQI}(c)$ \cite{ernst2005tree}}
    \label{algo:fqi}
    \begin{algorithmic}[1]
        \REQUIRE Collected data set $\D = \{ x_i,a_i,x_i^\prime,c_i\}_{i=1}^n$. Function class $\F$
        %\REQUIRE 
        \STATE Initialize $Q_0 \in \F$ randomly
        \FOR{$k = 1,2,\ldots,K$}
        %\REPEAT
        \STATE Compute target $y_i = c_i+\gamma\min_a Q_{k-1}(x_i^\prime,a) \enskip \forall i$ \\
        \STATE Build training set $\widetilde{\D}_k = \{(x_i,a_i),y_i \}_{i=1}^n$
        \STATE Solve a supervised learning problem: \\
        \quad $Q_k = \argmin\limits_{f\in\F} \frac{1}{n}\sum_{i=1}^n (f(x_i,a_i)-y_i )^2$
        %\UNTIL No improvement on validation set
        \ENDFOR
        \ENSURE $\pi_K(\cdot) = \argmin\limits_{a} Q_K(\cdot,a)$ (greedy policy with respect to the returned function $Q_K$)
    \end{algorithmic}
    \end{small}
\end{algorithm}
The analysis of Fitted Q Iteration (FQI) follows analogously from the analysis of FQE presented in the previous section (Appendix \ref{sec:proof-fqe}). For brevity, we skip certain detailed derivations, especially those that are largely identical to FQE's analysis. Algorithm \ref{algo:fqi} contains the pseudo-code for completeness. 

To the best of our knowledge, a finite-sample analysis of FQI with general non-linear function approximation has not been published. One can adapt existing analysis of fitted value iteration \cite{munos2008finite} and fitted policy iteration via Bellman residual minimization \cite{antos2008learning,antos2008fitted} to show that under similar assumptions, among policies greedy w.r.t. functions in $\F$, FQI will find $\epsilon-$ optimal policy using $n = \widetilde{O}(\frac{1}{\epsilon^4})$ samples. We derive an improved analysis of FQI with general non-linear function approximations, with better sample complexity of $n = \widetilde{O}(\frac{1}{\epsilon^2})$. We note that the appendix of \cite{lazaric2011transfer} contains an analysis of LinearFQI showing similar rate to ours, albeit with linear function approximators. 

%In this section, we prove the following statement for Fitted Q Iteration, mostly following the techniques from the proof of FQE in the previous section. To our knowledge, a finite-sample analysis of FQI has not been published. 
 %The full description of FQI and our proof are included in appendix \ref{sec:proof-fqi}.

In this section, we sketch the proof of the following statement:
\begin{thm}[Guarantee for FQI - General Case (theorem \ref{thm:fqi_main} in main paper)]
Under Assumption \ref{assume:concentrability}, for any $\epsilon>0, \delta\in(0,1)$, after $K$ iterations of Fitted Q Iteration (algorithm \ref{algo:fqi}), for $n=O\big(\frac{\widebar{C}^4}{\epsilon^2}( \log\frac{K}{\delta}+\pdim_{\F}\log\frac{\widebar{C}^2}{\epsilon^2}+\log \pdim_{\F})\big)$, we have with probability $1-\delta$:
$$C^*-C(\pi_K) \leq \frac{2\gamma}{(1-\gamma)^3}\big( \sqrt{\beta_{\mu}}\left(2d_\F+\epsilon\right) + 2\gamma^{K/2} \widebar{C}\big)$$
where $\pi_K$ is the policy greedy with respect to the returned function $Q_K$, and $C^*$ is the value of the optimal policy.
\end{thm}
The key steps to the proof follow similar scheme to the proof of FQE. We first bound the error for each iteration, and then analyze how the errors flow through the algorithm. 
\subsection{Single iteration error bound $\norm{Q_k-\T Q_{k-1}}_\mu$}
Here $\mu$ is the state-action distribution induced by the data-generating policy $\pi_\D$. For the Bellman (optimality) operator $\T$,  $\T Q_{k-1}$ is the \textit{regression function} that minimizes square loss $\min\limits_{h:\R^{X\times A}\mapsto\R}\E\abs{h(x,a)-y}^2$, with the random variables $(x,a)\sim\mu$ and $y=c(x,a)+\gamma\min_{a^\prime}Q_{k-1}(x^\prime,a^\prime)$ where $x^\prime\sim p(x^\prime|x,a)$.

\begin{prop}[Error bound for single iteration]\label{lem:single_iteration_bound} Let the functions in $\F$ be bounded by $\widebar{C}$, and let $\pdim_\F$ denote the pseudo-dimension of the function class $\F$. \\For $n\geq\frac{24\cdot214\cdot \widebar{C}^4}{\epsilon}\left( \log\frac{1}{\delta}+\pdim_\F\log\frac{320 \widebar{C}^2}{\epsilon}+\log(14e(\pdim_\F+1))\right)$:
$$\norm{Q_k-\T Q_{k-1}}_\mu^2 < \epsilon$$ with probability at least $1-\delta$.
\end{prop}
\begin{rem}
Note from proposition \ref{lem:single_iteration_bound} that the dependence of sample complexity $n$ here on $\epsilon$ is $\Tilde{O}(\frac{1}{\epsilon})$, which is much better than previously known analysis for Fitted Q Iteration dependence of $O(\frac{1}{\epsilon^2})$ \cite{antos2008fitted}. Note also that the Fitted Q Iteration algorithm from \cite{antos2008fitted} was proposed for continuous action space and thus is different from the FQI algorithm as presented in Algorithm \ref{algo:fqi}.
\end{rem}
We first bound the distance $\norm{Q_k-\T Q_{k-1}}_\mu$, where $\mu$ is the training distribution that generates the data set. Recall the training target is round $k$ is $y_i = c_i+\gamma\min_{a} Q_{k-1}(x_i^\prime, a)$ for $i=1,2,\ldots,n$, and $Q_k\in\F$ is the solution to the following regression problem:
\begin{equation}
    Q_k = \argmin_{f\in\F}\frac{1}{n}\sum_{i=1}^n (f(x_i,a_i)-y_i)^2
\end{equation}
Consider random variables $(x,a)\sim\mu$ and $y=c(x,a)+\gamma\min_{a^\prime}Q_{k-1}(x^\prime,a^\prime)$ where $x^\prime\sim p(x^\prime|x,a)$.
By this definition, $\T Q_{k-1}$ is the \textit{regression function} that minimizes square loss $\min\limits_{h:\R^{X\times A}\mapsto\R}\E\abs{h(x,a)-y}^2$ out of all functions $h$ (not necessarily in $\F$). This is due to $(\T Q_{k-1})(\tilde{x},\tilde{a}) = \E\left[y|x=\tilde{x},a=\tilde{a} \right]$ by definition of the Bellman operator. Consider $Q_{k-1}$ fixed and we now want to relate the learned function $Q_k$ over finite set of $n$ samples with the regression function over the whole data distribution via uniform deviation bound. 
\begin{lem}[\cite{gyorfi2006distribution}, theorem 11.4. Original version \cite{lee1996efficient}, theorem 3]\label{lem:bartlett} Consider random vector $(X,Y)$ and $n$ i.i.d samples $(X_i,Y_i)$. Let $m(x)$ be the (optimal) regression function under square loss $m(x) = \E[Y|X=x]$. Assume $\abs{Y}\leq B$ a.s. and $B\leq 1$. Let $\F$ be a set of function $f:\R^d\mapsto\R$ and let $\abs{f(x)}\leq B$. Then for each $n\geq 1$
\begin{align*}
    \mathbf{P}\bigg\{ \exists f\in\F: \E\abs{f(X)-Y}^2-\E\abs{m(X)-Y}^2 -\frac{1}{n}\sum_{i=1}^n\left( \abs{f(X_i)-Y_i}^2-\abs{m(X_i)-Y_i}^2\right) \geq \\ \epsilon\cdot\left(\alpha+\beta+\E\abs{f(X)-Y}^2-\E\abs{m(X)-Y}^2 \right) \bigg\} \\
    \leq 14\sup_{x_1^n}\mathcal{N}_1\left(\frac{\beta\epsilon}{20B},\F,x_1^n \right)\exp{\left(-\frac{\epsilon^2(1-\epsilon)\alpha n}{214(1+\epsilon)B^4}\right)}   
\end{align*}
where $\alpha,\beta>0$ and $0<\epsilon<1/2$
\end{lem}
To apply this lemma, first note that since $\T Q_{k-1}$ is the optimal regression function, we have
\begin{align}
    \E\left[(Q_k(x,a)-y)^2\right] &= \E\left[\left(Q_k(x,a)-\T Q_{k-1}(x,a) + \T Q_{k-1}(x,a) -y\right)^2\right] \\
    &=\E\left[\left(Q_k(x,a)-\T Q_{k-1}(x,a)\right)^2] + \E[\left(\T Q_{k-1}(x,a)-y\right)^2\right]
\end{align}
thus $\norm{Q_k-\T Q_{k-1}}_\mu^2 = \E\left[ (Q_k(x,a) - y)^2\right] - \E\left[ (\T Q_{k-1}(x,a)-y)^2\right]$ where $$\E\left[ (Q_k(x,a)-\T Q_{k-1}(x,a))^2\right] = \int\left(Q_k(x,a) - \T Q_{k-1}(x,a)\right)^2\mu(dx,a)$$
Next, given a fixed data set $D_k\sim\mu$
\begin{align}
    &\mathbf{P}\big\{ \norm{Q_k-\T Q_{k-1}}_\mu^2 > \epsilon \big\} = \mathbf{P}\bigg\{ \E\left[ (Q_k(x,a) - y)^2\right] - \E\left[ (\T Q_{k-1}(x,a)-y)^2\right] > \epsilon \bigg\} \\
    & \leq \mathbf{P}\bigg\{ \E\left[ (Q_k(x,a) - y)^2\right] - \E\left[ (\T Q_{k-1}(x,a)-y)^2\right] \nonumber\\
    &\qquad\qquad- 2\cdot\left(\frac{1}{n}\sum_{i=1}^n (Q_k(x_i,a_i)-y_i)^2 - \frac{1}{n}\sum_{i=1}^n(\T Q_{k-1}(x_i,a_i)-y_i)^2 \right) >\epsilon \bigg\} \label{eqn:relax_best_in_class}\\
    &=\mathbf{P}\bigg\{\E\left[ (Q_k(x,a)-y)^2\right] -\E\left[ (\T Q_{k-1}(x,a)-y)^2\right] \nonumber\\
    &\qquad\qquad-\frac{1}{n}\sum_{i=1}^n\left[ (Q_k(x_i,a_i)-y_i)^2-(\T Q_{k-1}(x_i,a_i)-y_i)^2\right]\nonumber\\
    &\qquad\qquad\qquad>\frac{1}{2}(\epsilon+\E\left[(Q_k(x,a)-y)^2 \right] -\E\left[(\T Q_{k-1}(x,a)-y)^2 \right])\bigg\} \label{eqn:rearrange_11_4}\\
    &\leq\mathbf{P} \bigg\{ \exists f\in\F: \E\left[(f(x,a)-y)^2\right]-\E\left[ (\T Q_{k-1}(x,a)-y)^2\right] \nonumber\\
    &\qquad\qquad-\frac{1}{n}\sum_{i=1}^n\left[ (f(x_i,a_i)-y_i)^2-(\T Q_{k-1}(x_i,a_i)-y_i)^2\right]\nonumber \\
    &\qquad\qquad\qquad \geq \frac{1}{2}(\frac{\epsilon}{2}+\frac{\epsilon}{2}+\E\left[(f(x,a)-y)^2\right]-\E\left[(\T Q_{k-1}(x,a)-y)^2\right] )\bigg\} \label{eqn:turn_functional_concentration}\\
    &\leq 14\sup_{x_1^n}\mathcal{N}_1\left(\frac{\epsilon}{80\widebar{C}},\F,x_1^n\right)\cdot\exp{\left(-\frac{n\epsilon}{24\cdot214\widebar{C}^4}\right)}\label{eqn:cover_bound}
\end{align}
Equation \ref{eqn:relax_best_in_class} uses the definition of $Q_k = \argmin\limits_{f\in\F}\frac{1}{n}\sum_{i=1}^n (f(x_i,a_i)-y_i)^2$ and the fact that $\T Q_{k-1}\in\F$, thus making the extra term a positive addition. Equation \ref{eqn:rearrange_11_4} is due to rearranging the terms. Equation \ref{eqn:cover_bound} is an application of lemma \ref{lem:bartlett}. We can further bound the empircal covering number by invoking the following lemma due to Haussler \cite{haussler1995sphere}:
% \begin{lem}[\cite{haussler1995sphere}, Corollary 3]\label{lem:haussler} For any set $X$, any points $x^{1:n}\in\X^n$, any class $\F$ of functions on $X$ taking values in $[0,B]$ with pseudo-dimension $\pdim_\F<\infty$, and any $\epsilon>0$
% $$\mathcal{N}_1(\epsilon, \F, x_1^n)\leq e(\pdim_\F+1)\left(\frac{2eB}{\epsilon}\right)^{\pdim_\F}$$

% \end{lem}
Applying lemma \ref{lem:haussler} to equation \ref{eqn:cover_bound}, we have that
\begin{equation}
\label{eqn:fqi_single_bound_realize}
    \mathbf{P}\big\{ \norm{Q_k-\T Q_{k-1}}_\mu^2 > \epsilon \big\} \leq 14\cdot e\cdot (\pdim_\F+1)\left( \frac{320 \widebar{C}^2}{\epsilon}\right)^{\pdim_\F}\cdot\exp{\left(-\frac{n\epsilon}{24\cdot214\widebar{C}^4}\right)}
\end{equation}
We thus have that when $n\geq\frac{24\cdot214\cdot \widebar{C}^4}{\epsilon}\left( \log\frac{1}{\delta}+\pdim_\F\log\frac{320 \widebar{C}^2}{\epsilon}+\log(14e(\pdim_\F+1))\right)$:
$$\norm{Q_k-\T Q_{k-1}}_\mu^2 < \epsilon$$ with probability at least $1-\delta$.
Notice that the dependence of sample complexity here on $\epsilon$ is $\Tilde{O}(\frac{1}{\epsilon})$, which is much better than previously known analysis for Fitted Q Iteration dependence of $O(\frac{1}{\epsilon^2})$ \cite{antos2008fitted}.
\subsection{Error bound for single iteration - non-realizable setting}
Consider the decomposition
\begin{align}
    \norm{Q_k-\T Q_{k-1}}_\mu^2 &= \E\left[ (Q_k(x,a) - y)^2\right] - \E\left[ (\T Q_{k-1}(x,a)-y)^2\right] \nonumber\\
    &= \bigg\{ \E\left[ (Q_k(x,a) - y)^2\right] - \E\left[ (\T Q_{k-1}(x,a)-y)^2\right] \nonumber \\
    &\qquad\qquad- 2\cdot\left(\frac{1}{n}\sum_{i=1}^n (Q_k(x_i,a_i)-y_i)^2 - \frac{1}{n}\sum_{i=1}^n(\T Q_{k-1}(x_i,a_i)-y_i)^2 \right)\bigg\} \nonumber \\
    &\qquad\qquad+ \bigg\{ 2\cdot\left(\frac{1}{n}\sum_{i=1}^n (Q_k(x_i,a_i)-y_i)^2 - \frac{1}{n}\sum_{i=1}^n(\T Q_{k-1}(x_i,a_i)-y_i)^2 \right) \bigg\} \nonumber \\
    &=\texttt{component\_1} + \texttt{component\_2} \nonumber
\end{align}
Splitting the probability of error into two separate bounds.
%$$\mathbf{P}(\norm{Q_k-\T Q_{k-1}}_\mu^2 >\epsilon) \leq \mathbf{P}(\texttt{component\_1} >\epsilon/2) + \mathbf{P}(\texttt{component\_2} >\epsilon/2)$$
We saw from the previous section that 
\begin{equation}
    \mathbf{P}(\texttt{component\_1} >\epsilon/2) \leq 14\cdot e\cdot (\pdim_\F+1)\left( \frac{640 \widebar{C}^2}{\epsilon}\right)^{\pdim_\F}\cdot\exp{\left(-\frac{n\epsilon}{48\cdot214\widebar{C}^4}\right)} \label{eqn:non_realize_single_iteration_3}
\end{equation}
We no longer have $\texttt{component\_2} \leq 0$ since $\T Q_{k-1}\notin \F$. Let $f^* = \arginf\limits_{f\in\F}\norm{f-\T Q_{k-1}}_\mu^2$. Since $Q_k = \argmin\limits_{f\in\F} \frac{1}{n}\sum_{i=1}^n (f(x_i,a_i)-y_i )^2$, we can upper-bound \texttt{component\_2} by
$$\texttt{component\_2}\leq 2\cdot\left(\frac{1}{n}\sum_{i=1}^n (f^*(x_i,a_i)-y_i)^2 - \frac{1}{n}\sum_{i=1}^n(\T Q_{k-1}(x_i,a_i)-y_i)^2 \right)$$
Unlike random function $Q_k$, we can treat $f^*$ as a fixed function and use standard concentration inequalities to bound the empirical average from the expectation. Let random variable $z = ((x,a),y)$, $z_i = ((x_i,a_i),y_i), i=1,\ldots,n$ and let 
$$h(z) = (f^*(x,a)-y)^2 - (\T Q_{k-1}(x,a)-y)^2$$
We have $\abs{h(z)}\leq 4\widebar{C}^2$. We will derive a bound for $$\mathbf{P}\left(\frac{1}{n}\sum_{i=1}^n h(z_i)-\E h(z)>\frac{\epsilon}{4}+\E h(z) \right)$$using Bernstein inequality. First, using the relationship $h(z) = (f^*(x,a)+\T Q_{k-1}(x,a) - 2y)(f^*(x,a)-\T Q_{k-1}(x,a))$, we note that the variance of $h(z)$ can be bounded by a constant factor of $\E h(z)$, since
\begin{align}
    \mathbf{Var}(h(z))&\leq \E h(z)^2 \leq 16\widebar{C}^2\E\left[ (f^*(x,a) - \T Q_{k-1}(x,a))^2\right] \nonumber \\
    &=16 \widebar{C}^2\left(\E\left[(f^*(x,a)-y)^2 \right]-\E\left[(\T Q_{k-1}(x,a)-y)^2 \right] \right) \label{eqn:non_realize_single_iteration_1}\\
    &=16 \widebar{C}^2\E h(z) \label{eqn:non_realize_single_iteration_2}
\end{align}
Equation \ref{eqn:non_realize_single_iteration_1} stems from $\T Q_{k-1}$ being the optimal regression function. Now we can apply equation \ref{eqn:non_realize_single_iteration_2} and Bernstein inequality to obtain
\begin{align*}
    &\mathbf{P}\left(\frac{1}{n}\sum_{i=1}^n h(z_i)-\E h(z)>\frac{\epsilon}{4}+\E h(z) \right) \leq \mathbf{P} \left( \frac{1}{n}\sum_{i=1}^n h(z_i)-\E h(z)>\frac{\epsilon}{4}+ \frac{\mathbf{Var}(h(z))}{16\widebar{C}^2}\right) \leq \ldots\\
    &\leq \exp{\left( -\frac{n\left(\frac{\epsilon}{4} +\frac{\mathbf{Var}}{16\widebar{C}^2} \right)^2 }{2\mathbf{Var}+2\frac{4\widebar{C}^2}{3}\left( \frac{\epsilon}{4} + \frac{\mathbf{Var}}{16\widebar{C}^2}\right)  } \right)} \\
    &\leq \exp{\left( -\frac{n\left(\frac{\epsilon}{4} +\frac{\mathbf{Var}}{16\widebar{C}^2} \right)^2 }{ \left(32\widebar{C}^2+\frac{8\widebar{C}^2}{3}\right) \left( \frac{\epsilon}{4} + \frac{\mathbf{Var}}{16\widebar{C}^2}\right)  } \right)} = \exp{\left( -\frac{n\left(\frac{\epsilon}{4} +\frac{\mathbf{Var}}{16\widebar{C}^2} \right) }{ 32\widebar{C}^2+\frac{8\widebar{C}^2}{3}  } \right)} \leq \exp{\left(-\frac{1}{128+\frac{32}{3}}\cdot\frac{n\epsilon}{\widebar{C}^2} \right)}
\end{align*}
%\begin{align*}
%    &\mathbf{P}\left(\frac{1}{n}\sum_{i=1}^n h(z_i)-\E h(z)>\frac{\epsilon}{4}+\E h(z) \right) \\
%    &\leq \mathbf{P} \left( \frac{1}{n}\sum_{i=1}^n h(z_i)-\E h(z)>\frac{\epsilon}{4}+ \frac{\mathbf{Var}(h(z))}{16\widebar{C}^2}\right) \\
%    &\leq \exp{\left( -\frac{n\left(\frac{\epsilon}{4} +\frac{\mathbf{Var}}{16\widebar{C}^2} \right)^2 }{2\mathbf{Var}+2\frac{4\widebar{C}^2}{3}\left( \frac{\epsilon}{4} + \frac{\mathbf{Var}}{16\widebar{C}^2}\right)  } \right)} \\
%    &\leq \exp{\left( -\frac{n\left(\frac{\epsilon}{4} +\frac{\mathbf{Var}}{16\widebar{C}^2} \right)^2 }{ \left(32\widebar{C}^2+\frac{8\widebar{C}^2}{3}\right) \left( \frac{\epsilon}{4} + \frac{\mathbf{Var}}{16\widebar{C}^2}\right)  } \right)} = \exp{\left( -\frac{n\left(\frac{\epsilon}{4} +\frac{\mathbf{Var}}{16\widebar{C}^2} \right) }{ 32\widebar{C}^2+\frac{8\widebar{C}^2}{3}  } \right)} \\
%    &\leq \exp{\left(-\frac{1}{128+\frac{32}{3}}\cdot\frac{n\epsilon}{\widebar{C}^2} \right)}
%\end{align*}

Thus
\begin{equation}
\mathbf{P}\left( 2\cdot\left[\frac{1}{n}\sum_{i=1}^n h(z_i) - 2\E h(z)\right] >\frac{\epsilon}{2}\right) \leq \exp{\left(-\frac{3}{416}\cdot\frac{n\epsilon}{\widebar{C}^2}\right)}
    \label{eqn:non_realize_single_iteration_4}
\end{equation}
Now we have $$\texttt{component\_2}\leq 2\cdot\frac{1}{n}\sum_{i=1}^n h(z_i) = 2\cdot\left[\frac{1}{n}\sum_{i=1}^n h(z_i) - 2\E h(z)\right] + 4\E h(z)$$
Again using the fact that $\T Q_{k-1}$ is the optimal regression function
\begin{align}
    \E h(z) &= \E_D\left[ (f^*(x,a)-y)^2\right]-\E_D\left[ (\T Q_{k-1}(x,a)-y)^2\right] = \E_D\left[ (f^*(x,a) - \T Q_{k-1}(x,a))^2\right] \nonumber \\
    &= \inf_{f\in\F}\norm{f-\T Q_{k-1}}_\mu^2 \label{eqn:non_realize_single_iteration_5}
\end{align}
Combining equations (\ref{eqn:non_realize_single_iteration_3}), (\ref{eqn:non_realize_single_iteration_4}) and (\ref{eqn:non_realize_single_iteration_5}), we can conclude that 
\begin{align}
    \mathbf{P}\big\{ \norm{Q_k-\T Q_{k-1}}_\mu^2-4\inf_{f\in\F}\norm{f-\T Q_{k-1}}_\mu^2 > \epsilon \big\} &\leq  14\cdot e\cdot (\pdim_\F+1)\left( \frac{640 \widebar{C}^2}{\epsilon}\right)^{\pdim_\F}\cdot\exp{\left(-\frac{n\epsilon}{48\cdot214\widebar{C}^4}\right)} \nonumber \\ 
    &\qquad +\exp{\left(-\frac{3}{416}\cdot\frac{n\epsilon}{\widebar{C}^2}\right)} \label{eqn:non_realize_single_iteration_6}
\end{align}
The term $4\inf_{f\in\F}\norm{f-\T Q_{k-1}}_\mu^2 \leq 4\sup_{f^\prime\in\F}\inf_{f\in\F}\norm{f-\T f^\prime}_\mu^2$ essentially reflects the \textit{inherent Bellman error}. Unfortunately, this inherent Bellman error cannot generally be estimated (see counter-examples from section 11.6 of \cite{sutton2018reinforcement}). In principle, inherent Bellman error can be driven to be small by choosing rich function class $\F$ (low bias), at the expense of more samples requirement (high variance, through for example higher pseudo-dimension $V_\F$).

While the bound in (\ref{eqn:non_realize_single_iteration_6}) certainly looks more complicated than the realizable case, note that the convergence rate will still be $O(\frac{1}{n})$, which is an improvement over previously known rate of $O(\frac{1}{n^2})$ in related approximate dynamic programming algorithms \cite{antos2008fitted, antos2008learning, munos2008finite}. The only previously known rate of $O(\frac{1}{n})$ was for linear function approximation case for LSPI \cite{lazaric2012finite} and linear Fitted-Q-Iteration \cite{lazaric2011transfer}. Here we provide the same convergence rate for general non-linear function approximators. 
\subsection{Propagation of error bound}
The proof largely follows the error propagation analysis in lemma 3 and 4 of \cite{munos2008finite} in the fitted value iteration context (for $V$ function). We include the $Q$ function derivation here for completeness. 

Let $\pi_K$ be the greedy policy wrt the learned function $Q_K$ returned by the Fitted Q Iteration procedure in algorithm \ref{algo:fqi}. Our overall goal is to bound the difference $V^*-V^{\pi_K}$ between the optimal value function and that of the returned policy $\pi_K$. We first bound the loss $\norm{Q^*-Q^{\pi_K}}_{\rho}$ under any distribution $\rho$ of $(x,a)$ different from the data generating distribution $\mu$. 

\textbf{Step 1: Upper-bound the propagation error (value)}. Let $\epsilon_{k-1} = Q_k - \T Q_{k-1}$. We have that 
\begin{align}
    Q^* - Q_k &= \T^{\pi^*}Q^*-\T^{\pi^*}Q_{k-1}+\T^{\pi^*}Q_{k-1}-\T Q_{k-1}+\epsilon_{k-1} \nonumber\\
    &\leq \T^{\pi^*}Q^*-\T^{\pi^*}Q_{k-1} + \epsilon_{k-1} \qquad\qquad\text{ (since } \T Q_{k-1}\geq \T^{\pi^*} Q_{k-1}\text{)} \nonumber\\
    &=\gamma P^{\pi^*}(Q^*-Q_{k-1})+\epsilon_{k-1}\nonumber
\end{align}
Thus by recursion
\begin{equation}
\label{eqn:propagation_upper_bound}
 Q^*-Q_K\leq \sum_{k=0}^{K-1}\gamma^{K-k-1}(P^{\pi^*})^{K-k-1}\epsilon_k + \gamma^K (P^{\pi^*})^K(Q^*-Q_0)   
\end{equation}

\textbf{Step 2: Lower-bound the propagation error (value)}. Similarly
\begin{align}
    Q^*-Q_k &= \T Q^*-\T^{\pi_{k-1}}Q^*+\T^{\pi_{k-1}}Q^*-\T Q_{k-1}+\epsilon_{k-1} \nonumber \\
    &\geq \T^{\pi_{k-1}}Q^*-\T Q_{k-1} +\epsilon_{k-1} \qquad\qquad\text{ (since } \T Q^*\geq \T^{\pi_{k-1}} Q^*\text{)} \nonumber\\
    &\geq \T^{\pi_{k-1}}Q^*-\T^{\pi_{k-1}}Q_{k-1}+\epsilon_{k-1} \qquad\qquad\text{ (since } \pi_{k-1}\text{ greedy wrt }Q_{k-1}) \nonumber\\
    &=\gamma P^{\pi_{k-1}}(Q^*-Q_{k-1}) +\epsilon_{k-1}\nonumber
\end{align}
Thus by recursion 
\begin{equation}
 \label{eqn:propagation_lower_bound}
 Q^*-Q_K\geq \sum_{k=0}^{K-1} \gamma^{K-k-1}(P^{\pi_{K-1}}P^{\pi_{K-2}}\ldots P^{\pi_{k+1}})\epsilon_k + \gamma^K(P^{\pi_{K-1}}P^{\pi_{K-2}}\ldots P^{\pi_0})(Q^*-Q_0)
\end{equation}
\textbf{Step 3: Upper-bound the propagation error (policy)}. Beginning with a decomposition of value wrt to policy $\pi_K$
\begin{align}
    Q^*-Q^{\pi_K} &= \T^{\pi^*}Q^*-\T^{\pi^*}Q_K+\T^{\pi^*}Q_K-\T^{\pi_K}Q_K+\T^{\pi_K}Q_K-\T^{\pi_K}Q^{\pi_K} \nonumber\\
    &\leq (\T^{\pi^*}Q^*-\T^{\pi^*}Q_K)+(\T^{\pi_K}Q_K-\T^{\pi_K}Q^{\pi_K}) \qquad (\text{ since }\T^{\pi^*}Q_K\leq \T Q_K = \T^{\pi_K}Q_K) \nonumber\\
    &=\gamma P^{\pi^*}(Q^*-Q_K)+\gamma P^{\pi_K}(Q_K-Q^{\pi_K}) \nonumber\\
    &=\gamma P^{\pi^*}(Q^*-Q_K)+\gamma P^{\pi_K}(Q_K-Q^*+Q^*-Q^{\pi_K})\nonumber
\end{align}
Thus leading to $$(I-\gamma P^{\pi_K})(Q^*-Q^{\pi_K})\leq \gamma(P^{\pi^*}-P^{\pi_K})(Q^*-Q_K)$$
Operator $(I-\gamma P^{\pi_K})$ is invertible and $(I-\gamma P^{\pi_K})^{-1} = \sum_{m\geq0}\gamma^m(P^{\pi_K})^m$ is monotonic. Thus
\begin{align}
    Q^*-Q^{\pi_K}&\leq \gamma(I-\gamma P^{\pi_K})^{-1}(P^{\pi^*}-P^{\pi_K})(Q^*-Q_K) \nonumber \\
    &=\gamma(I-\gamma P^{\pi_K})^{-1}P^{\pi^*}(Q^*-Q_K)- \gamma(I-\gamma P^{\pi_K})^{-1}P^{\pi_K}(Q^*-Q_K)\label{eqn:propagation_1}
\end{align}
Applying inequalities \ref{eqn:propagation_upper_bound} and \ref{eqn:propagation_lower_bound} to the RHS of \ref{eqn:propagation_1}, we have
\begin{align}
    Q^*-Q^{\pi_K}\leq (I-\gamma P^{\pi_K})^{-1}\bigg[&\sum_{k=0}^{K-1}\gamma^{K-k}\left( (P^{\pi^*})^{K-k}-P^{\pi_K}P^{\pi_{K-1}}\ldots P^{\pi_{k+1}} \right)\epsilon_k \nonumber \\
    &+\gamma^{K+1}\left( (P^{\pi^*})^{K+1} - (P^{\pi_K}P^{\pi_{K-1}}\ldots P^{\pi_0}) \right) (Q^*-Q_0)\bigg] \label{eqn:propagation_2}
\end{align}
We can apply point-wise absolute value on RHS of (\ref{eqn:propagation_2}) with $\abs{\epsilon_k}$ being the short-hand notation for $\abs{\epsilon_k(x,a)}$ point-wise. Using triangle inequalities and rewriting (\ref{eqn:propagation_2}) in a more compact form (\cite{munos2008finite}):
\begin{equation*}
    Q^*-Q^{\pi_K}\leq \frac{2\gamma(1-\gamma^{K+1})}{(1-\gamma)^2}\left[\sum_{k=0}^{K-1}\alpha_k A_k \abs{\epsilon_k}+\alpha_K A_K \abs{Q^*-Q_0} \right]
\end{equation*}
where
\begin{align*}
    \alpha_k &= \frac{(1-\gamma)\gamma^{K-k-1}}{1-\gamma^{K+1}} \text{ for }k<K, \alpha_K = \frac{(1-\gamma)\gamma^K}{1-\gamma^{K+1}} \nonumber \\
    A_k &= \frac{1-\gamma}{2}(I-\gamma P^{\pi_K})^{-1}\left[(P^{\pi^*})^{K-k}+ P^{\pi_K}P^{\pi_{K-1}}\ldots P^{\pi_{k+1}}\right] \text{ for } k<K \nonumber \\
    A_K &= \frac{1-\gamma}{2}(I-\gamma P^{\pi_K})^{-1}\left[(P^{\pi^*})^{K+1}+ P^{\pi_K}P^{\pi_{K-1}}\ldots P^{\pi_{0}}\right]\nonumber
\end{align*}
Note that $A_k$'s are probability kernels that combine the $P^{\pi_i}$ terms and $\alpha_k$'s are chosen such that $\sum_k \alpha_k = 1$.

\textbf{Step 4: Bounding $\norm{Q^*-Q^{\pi_K}}_\rho^2$ for any test distribution $\rho$}. To handle distribution shift from $\mu$ to $\rho$:
\begin{align}
    \norm{Q^*-Q^{\pi_K}}_\rho^2&=\int\rho(dx,da)\left(Q^*(x,a)-Q^{\pi_K}(x,a) \right)^2 \nonumber \\
    &\leq \left[ \frac{2\gamma(1-\gamma^{K+1})}{(1-\gamma)^2}\right]^2\int\rho(dx,da)\left[\sum_{k=0}^{K-1}\alpha_k A_k\abs{\epsilon_k}+\alpha_K A_K\abs{Q^*-Q_0} \right]^2(x,a) \text{ (Jensen)}\nonumber\\
    &\leq \left[ \frac{2\gamma(1-\gamma^{K+1})}{(1-\gamma)^2}\right]^2\int\rho(dx,da)\left[\sum_{k=0}^{K-1}\alpha_k A_k \epsilon_k^2+\alpha_K A_K(Q^*-Q_0)^2 \right](x,a) \text{ (Jensen)}\nonumber
\end{align}
Using assumption \ref{assume:concentrability}, we can bound each term $\rho A_k$ as 
\begin{align}
    \rho A_k &= \frac{1-\gamma}{2}\rho (I-\gamma P^{\pi_K})^{-1}\left[(P^{\pi^*})^{K-k}+P^{\pi_K}P^{\pi_{K-1}}\ldots P^{\pi_{k+1}} \right] \nonumber\\
    &=\frac{1-\gamma}{2}\sum_{m\geq0}\gamma^m \rho(P^{\pi_K})^m \left[(P^{\pi^*})^{K-k}+P^{\pi_K}P^{\pi_{K-1}}\ldots P^{\pi_{k+1}} \right] \nonumber\\
    &\leq (1-\gamma)\sum_{m\geq0} \gamma^m \beta_\mu(m+K-k)\mu \qquad \text { (definition \ref{def:concentrability})}
\end{align}
Thus
\begin{align}
    \norm{Q^*-Q^{\pi_K}}_\rho^2 &\leq \left[ \frac{2\gamma(1-\gamma^{K+1})}{(1-\gamma)^2}\right]^2 \left[\frac{1}{1-\gamma^{K+1}}\sum_{k=0}^{K-1} (1-\gamma)^2\sum_{m\geq0} \gamma^{m+K-k-1} \beta_\mu(m+K-k)\norm{\epsilon_k}_\mu^2 +\alpha_K(2\widebar{C})^2 \right] \nonumber \\
    &\leq \left[ \frac{2\gamma(1-\gamma^{K+1})}{(1-\gamma)^2}\right]^2 \left[ \frac{1}{1-\gamma^{K+1}} \beta_\mu \max_{k}\norm{\epsilon_k}_\mu^2 +\alpha_K (2\widebar{C})^2  \right] \qquad \text{(assumption \ref{assume:concentrability})}\nonumber \\
    %&= \left[ \frac{2\gamma(1-\gamma^{K+1})}{(1-\gamma)^2}\right]^2 \left[(1-\alpha_K)\beta_\mu\max_k\norm{\epsilon_k}_\mu^2 + \alpha_K(2\widebar{C})^2 \right] \nonumber \\
    &= \left[ \frac{2\gamma(1-\gamma^{K+1})}{(1-\gamma)^2}\right]^2 \left[\frac{1}{1-\gamma^{K+1}}\beta_\mu\max_k\norm{\epsilon_k}_\mu^2 + \frac{(1-\gamma)\gamma^K}{1-\gamma^{K+1}}(2\widebar{C})^2 \right] \nonumber \\
    &\leq \left[ \frac{2\gamma(1-\gamma^{K+1})}{(1-\gamma)^2}\right]^2 \left[\frac{1}{1-\gamma^{K+1}}\beta_\mu\max_k\norm{\epsilon_k}_\mu^2 + \frac{\gamma^K}{1-\gamma^{K+1}}(2\widebar{C})^2 \right] \nonumber \\
    &\leq\left[\frac{2\gamma}{(1-\gamma)^2} \right]^2 \left[\beta_\mu\max_{k}\norm{\epsilon_k}_\mu^2 + \gamma^K(2\widebar{C})^2 \right]
    %&\leq \left[\frac{2\gamma}{(1-\gamma)^2}\sqrt{\beta_\mu}\max_{k}\norm{\epsilon}_\mu +  \right] \\
    %&\leq \left[ \frac{2\gamma}{(1-\gamma)^2}\right]^2 \beta_\mu \max_k \norm{\epsilon_k}_{\mu}^2
\end{align}
Using $a^2+b^2\leq(a+b)^2$ for nonnegative $a,b$, we thus conclude that
\begin{equation}
\label{eqn:error_propagation_bound}
    \norm{Q^* - Q^{\pi_K}}_\rho \leq \frac{2\gamma}{(1-\gamma)^2} \left( \sqrt{\beta_\mu}\max_k\norm{\epsilon_k}_\mu + 2\gamma^{K/2} \widebar{C}\right)
\end{equation}
\textbf{Step 5: Bounding $V^*-V^{\pi_K}$}
Using the performance difference lemma (lemma 6.1 of \cite{kakade2002approximately}, which states that $V^*-V^{\pi_K} = -\frac{1}{1-\gamma}\E_{\substack{x\sim d_{\pi_K} \\ a\sim\pi_K}} A^*\left[x,a \right]$. We can upper-bound the performance difference of value function as
\begin{align}
    V^*-V^{\pi_K}  &= \frac{1}{1-\gamma}\E_{\substack{x\sim d_{\pi_K}\\a\sim \pi_K}} \left[ V^*(x) - Q^*(x,a)\right] \nonumber\\
    &= \frac{1}{1-\gamma}\E_{x~\sim d_{\pi_K}} \left[ V^*(x) - Q^*(x,\pi_K(x))\right] \nonumber \\
    &\leq \frac{1}{1-\gamma}\E_{x~\sim d_{\pi_K}} \left[ Q^*(x,\pi^*(x)) -Q_K(x,\pi^*(x)) + Q_K(x,\pi_K(x)- Q^*(x,\pi_K(x))\right] \text{(greedy)} \nonumber \\
    &\leq \frac{1}{1-\gamma}\E_{x~\sim d_{\pi_K}} \lvert Q^*(x,\pi^*(x)) -Q_K(x,\pi^*(x))\rvert + \lvert Q_K(x,\pi_K(x)- Q^*(x,\pi_K(x))\rvert \nonumber \\
    &\leq \frac{1}{1-\gamma} \left( \norm{Q^*-Q^{\pi_K}}_{d_{\pi_K}\times\pi^*}+\norm{Q^*-Q^{\pi_K}}_{d_{\pi_K}\times\pi_K} \right) \text{(upper-bound 1-norm by 2-norm)}\nonumber \\
    &\leq \frac{2\gamma}{(1-\gamma)^3}\left( \sqrt{\beta_\mu}\max_k\norm{\epsilon_k}_\mu + 2\gamma^{K/2} \widebar{C}\right) \label{eqn:fqi_v_bound_propagation}
\end{align}
\subsection{Finite-sample guarantees for Fitted Q Iteration}
Combining the derived results from (\ref{eqn:fqi_single_bound_realize}), (\ref{eqn:non_realize_single_iteration_6}) and (\ref{eqn:fqi_v_bound_propagation}), we have the final finite-sample analysis for Fitted Q Iteration under both realizable and non-realizable cases.

\textbf{Realizable Case.} From (\ref{eqn:fqi_single_bound_realize}),  when $n\geq\frac{24\cdot214\cdot \widebar{C}^4}{\epsilon^2}\left( \log\frac{K}{\delta}+\pdim_\F\log\frac{320 \widebar{C}^2}{\epsilon^2}+\log(14e(\pdim_\F+1))\right)$, we have
$\norm{\epsilon_k}_\mu < \epsilon$ with probability at least $1-\delta/K$ for any $0\leq k<K$. Thus we conclude that for any $\epsilon>0, 0<\delta<1$, after $K$ iterations of Fitted Q Iteration, and for $\pi_K$ the greedy policy wrt $Q_K$:
$$V^*-V^\pi_K \leq \frac{2\gamma}{(1-\gamma)^3}\left( \sqrt{\beta_\mu}\epsilon + 2\gamma^{K/2} \widebar{C}\right)$$
holds with probability $1-\delta$ when $n\geq\frac{24\cdot214\cdot \widebar{C}^4}{\epsilon^2}\left( \log\frac{K}{\delta}+\pdim_\F\log\frac{320 \widebar{C}^2}{\epsilon^2}+\log(14e(\pdim_\F+1))\right)$.

\textbf{Non-realizable Case.} Similarly, from (\ref{eqn:non_realize_single_iteration_6}) we have
\begin{align}
    \mathbf{P}\big\{ \norm{Q_k-\T Q_{k-1}}_\mu-2\inf_{f\in\F}\norm{f-\T Q_{k-1}}_\mu > \epsilon \big\} &\leq  14\cdot e\cdot (\pdim_\F+1)\left( \frac{640 \widebar{C}^2}{\epsilon^2}\right)^{\pdim_\F}\cdot\exp{\left(-\frac{n\epsilon^2}{48\cdot214\widebar{C}^4}\right)} \nonumber \\ 
    &\qquad +\exp{\left(-\frac{3}{416}\cdot\frac{n\epsilon^2}{\widebar{C}^2}\right)} \nonumber
\end{align}
Since $\inf_{f\in\F}\norm{f-\T Q_{k-1}}_\mu \leq\sup_{h\in\F}\inf_{f\in\F}\norm{f-\T h}_\mu = d(\F,\T\F)_\mu$ (defined as the \textit{inherent Bellman error} \cite{munos2008finite}), similar arguments to the realizable case lead to the conclusion that for any $\epsilon>0, 0<\delta<1$, after $K$ iterations of Fitted Q Iteration, and for $\pi_K$ the greedy policy wrt $Q_K$:
$$V^*-V^\pi_K \leq \frac{2\gamma}{(1-\gamma)^3}\left( \sqrt{\beta_\mu}(2d(\F,\T\F)+\epsilon) + 2\gamma^{K/2} \widebar{C}\right)$$
holds with probability $1-\delta$ when $n=\text{poly}(\frac{1}{\epsilon^2},\log\frac{K}{\delta}, V_\F, V_{\max})$.
 
 Note that in both cases, the $\widetilde{O}(\frac{1}{\epsilon^2})$ dependency of $n$ is significant improvement over previous finite-sample analysis of related approximate dynamic programming algorithms \cite{munos2008finite, antos2008learning, antos2008fitted}. This dependency matches that of previous analysis using linear function approximators from \cite{lazaric2012finite} for LSPI algorithm. Here our analysis, using similar assumptions, is applicable for general non-linear function classes.


 \iffalse
We first focus on the sample complexity guarantee of Fitted-Q-Iteration (FQI) procedure. The algorithm was originally proposed in \cite{ernst2005tree} without analysis. FQI was further experimentally validated to be a good off-policy learning algorithm by \cite{riedmiller2005neural}. Although some key ideas for analyzing closedly related algorithms exist in the literature, a final analysis of FQI with discrete action space in its original form has never been published to the best of our knowledge (The closest is LinearFQI algorithm with some proof in the appendix of \cite{lazaric2011transfer}). Some notable previous proofs include those for Approximate Value Iteration \cite{munos2008finite}, Approximate Policy Iteration \cite{munos2003error}, Fitted Policy Iteration with Q-function (called FittedPolicyQ) by \cite{antos2008learning}, of which LSPI (\cite{lagoudakis2003least}) is shown to be a special case, Fitted Q Iteration in continuous action space by \cite{antos2008fitted} (different algorithm from FQI). While it is possible to adapt proofs from previous work to analyze FQI, here we propose an improvement over previous attempts to improve the convergence rate from $O(n^{-4})$ to $O(n^{-2})$, where $n$ is the number of samples. A minor modification suffices to show similar convergence rate for Fitted Off-Policy Evaluation algorithm (FQE). To simplify the presentation, we will focus exclusively on $\ell_2$ norm loss and error bounds in both the algorithm and analysis. Note that the analysis for for general $p$-norm, $p\geq1$ is identical. 

First, recall some standard notations from reinforcement learning. The Bellman optimality operator $\T:\mathcal{B}(\X\times\A;V_{\text{max}})\mapsto\mathcal{B}(\X\times\A;V_{\text{max}})$ as 
\begin{equation}
    (\T Q)(x,a) = r(x,a) + \gamma\int_{\X}\max_{a^\prime\in\A} Q(x^\prime,a^\prime)p(x^\prime|x,a)dx^\prime
\end{equation}
The optimal value functions are defined in the usual manner by $V^*(x) = \sup\limits_{\pi}V^\pi(x)$ and $Q^*(x,a) = \sup\limits_{\pi} Q^\pi(x,a)\enskip\forall x\in\X, a\in\A$. The classic value iteration algorithm can be described compactly using the Bellman operator form $Q_{k+1} = \T Q_k$. Convergence proof in exact value iteration can be established by using a max-norm contraction argument over $\infty$-norm as $\norm{Q^*-Q_{k+1}}_\infty\leq\gamma\norm{Q^*-Q_k}_\infty$. The key issue in approximate dynamic programming is $Q_{k+1}\approx \T Q_k$, thus convergence may not be guaranteed (counter example proposed from \cite{tsitsiklis1996feature}). 

Similarly, the policy-based Bellman operator $\Tpi:\mathcal{B}(\X\times\A;V_{\text{max}})\mapsto\mathcal{B}(\X\times\A;V_{\text{max}})$ as 
\begin{equation}
    (\Tpi Q)(x,a) = r(x,a) + \gamma\int_{\X} Q(x^\prime,\pi(x^\prime))p(x^\prime|x,a)dx^\prime
\end{equation}
It is well known that $\Tpi Q^\pi = Q^\pi,$ a fixed point of the $\Tpi$ operator. 

Let us denote the data generating distribution as $\mu$, i.e $(x_i,a_i)\sim\mu$ for $(x_i,a_i,x_i^\prime, r_i)\in\D$. For each $(x_i,a_i)$, we have $x_i^\prime\sim p(\cdot|x_i,a_i)$ and $r_i=r(x_i,a_i)$. In the MDP setting, we can treat $\{ (x_i,a_i)\}$ as independent \hle{no? still need uniform over actions?}. For any (measurable) function $f:\X\times\A\mapsto\R$, define the $\mu$-weighted $\ell_2$ norm of $f$ as $\norm{f}_\mu^2 = \frac{1}{\abs{\A}}\sum\limits_{a\in\A}\int_{\X}f(x,a)^2\mu(dx)$.\hle{show that it's a norm} 

We begin with some standard definition and assumptions. First definition deals with approximation power of the policy class chosen. Specifically, to express how well the Bellman operator $\T g$ can be approximated by a function in the policy class $\F$, when $\T g\notin\F$, a notion of distance, known as inherent Bellman error is needed (\cite{munos2008finite}).
\begin{defn}[Inherent Bellman Error] Given a function class $\F$, the \textit{inherent Bellman error} of $\F$ is defined as
\begin{equation*}
    d(\F,\T\F) = \sup_{g\in\F}\inf_{f\in\F}\norm{f-\T g}
\end{equation*}
where $\norm{\cdot}$ is defined over certain distribution of input.
\end{defn}
We will assume the selection of a sufficiently rich function class so that the inherent Bellman error is 0. This is equivalent to realizability of the Bellman operator with respect to the policy class under consideration. This assumption also significantly simplifies the presentation of our bounds and simplifies the final error analysis of algorithm \ref{algo:main_algo}. After analyzing FQI under this realizability assumption, we will show the error bound under settings where the Bellman operator is not realizable.
\begin{assumption}
We consider function classes $\F$ sufficiently rich so that $d(\T \F,\F) =0$
\end{assumption}

Let $P^\pi$ denote the operator acting on $f:\X\times\A\mapsto\R$ such that $(P^\pi f)(x,a) = \int_\X f(x^\prime, \pi(x^\prime)) p(x^\prime|x,a) dx^\prime$. Next, we present a definition and two standard assumptions in the analysis of approximate dynamic programming algorithms \cite{lazaric2012finite, munos2008finite, antos2008fitted}. Since most value or policy-based iteration algorithms in multiple rounds, policy learned during each round will induce a different stationary state distribution. We want to have a way to quantify how much the induced state distribution shifts throughout the learning process. 

\begin{defn}[Concentration coefficient of state-action distribution]\label{def:concentrability} Given $\mu, \rho, m \geq 0$ and an arbitrary sequence of stationary policies $\{ \pi_m\}_{m\geq 1}$ let 
\begin{equation*}
c_{\rho, \mu}(m) = \sup_{\pi_1,\ldots,\pi_m} \left\| \frac{d(\rho P^{\pi_1}P^{\pi_2}\ldots P^{\pi_m})}{d\mu} \right\|_\infty    
\end{equation*}
($c^\pi_{\rho, \mu}(m) = \infty$ if the future state distribution $\rho P^{\pi_1}P^{\pi_2}\ldots P^{\pi_m}$ is not absolutely continuous w.r.t. $\mu$, i.e, $\rho P^{\pi_1}P^{\pi_2}\ldots P^{\pi_m}(x,a)>0$ for some $\mu(x,a) = 0$)
\end{defn}
\fi 

